Radial pulsations of gravitationally decoupled anisotropic self-bound stars with a generalized linear equation of state

We construct anisotropic self-bound stellar configurations through gravitational decoupling in the minimal geometric deformation framework and investigate their stability against linear radial perturbations. Retaining the Tolman IV temporal potential, we impose the generalized linear equation of state $P_r=\eta(\rho-\rho_s)$ on the complete matter distribution. Central regularity and Schwarzschild matching determine the radial geometry and relate the surface density to the compactness and stellar radius. Closed-form solutions are obtained for $\eta=1,1/2,1/3,1/4$, including the MIT bag radial relation when $\eta=1/3$ and $\rho_s=4B$. Since the equilibrium anisotropy does not determine its dynamical response, we introduce two material prescriptions that preserve either the anisotropy of each fluid layer or its ratio to $\rho+P_r$. Including metric perturbations, we compute the fundamental mode and three overtones for twelve equilibrium configurations under both prescriptions. All 24 background response combinations have positive fundamental squared frequencies, establishing linear radial stability within the adopted closures. The fundamental eigenvalue decreases with compactness within each sampled family, while changing the anisotropic response produces shifts whose direction depends on the background. Tangential tensions in several configurations and the failed tangential profile diagnostic of the maximally stiff family limit their physical interpretation. These results provide analytically tractable self-bound backgrounds and demonstrate that identical equilibrium configurations can support distinct radial spectra depending on their anisotropic material response.

==> pulsations_individual.tex <==
\section{Radial pulsations of the self-bound configurations}
\label{rpnum:section}
\label{section-radial-pulsations}

We now investigate the linear radial response of the twelve equilibrium
configurations considered above. A static anisotropy profile does not specify
how the anisotropic stress responds to a displacement of the fluid. We therefore
state the material response explicitly and compare two closures that reproduce
the same equilibrium. The resulting stability statements refer to these
closures. This distinction is particularly relevant when the tangential
pressure remains nonzero at the surface, as in radial-stability studies of
anisotropic strange stars~\cite{arbanil2016anisotropic}.

\subsection{Material response and perturbation equations}
\label{rpnum:closure}

Let $\xi(r)e^{i\omega t}$ denote the radial displacement and let $\Delta_L$
and $\delta$ denote Lagrangian and Eulerian perturbations, respectively, so
that $\Delta_L F=\delta F+\xi\,dF/dr$. The equilibrium parameters $\eta$ and
$\rho_s$ are held fixed during each oscillation. Consequently,
\begin{equation}
 \Delta_L P_r=\eta\,\Delta_L\rho.
 \label{rpnum:perturbed-eos}
\end{equation}
Writing $\Sigma=P_t-P_r$ for the physical anisotropy, we introduce a material
label $a_L$ that is transported with each fluid layer and prescribe
\begin{equation}
 \Sigma(a_L,\rho)=\Sigma_0(a_L)
 \left[\frac{\rho+P_r}{\rho_0(a_L)+P_{r0}(a_L)}\right]^\kappa,
 \qquad \kappa=0,1.
 \label{rpnum:material-law}
\end{equation}
The subscript $0$ denotes the chosen background. For $\kappa=0$, each layer
preserves its anisotropy, whereas for $\kappa=1$ it preserves
$\Sigma/(\rho+P_r)$. These are phenomenological response laws; they are not
deduced from the equilibrium equation of state or from gravitational
decoupling. Both preserve the central behavior $\Sigma=O(r^2)$ on the regular
perturbative branch. Their linearization gives
\begin{equation}
 \Delta_L\Sigma=
 \frac{\kappa(1+\eta)\Sigma}{\eta(\rho+P_r)}\Delta_LP_r.
 \label{rpnum:anisotropy-response}
\end{equation}
In particular, $\Delta_L\Sigma=0$ and $\delta\Sigma=0$ are different
prescriptions.

For the numerical problem we use $x=r/R$, $H=e^{-\lambda}$,
$b=e^\nu=1-3u+ux^2$, and the dimensionless background variables
\begin{equation}
 \begin{aligned}
 \varepsilon&=8\pi R^2\rho,& p&=8\pi R^2P_r,\\
 \sigma&=8\pi R^2(P_t-P_r),& w&=\varepsilon+p.
 \end{aligned}
 \label{rpnum:background-variables}
\end{equation}
The factors in Eq.~\eqref{rpnum:background-variables} use geometrized units,
$G=c=1$. We define
\begin{equation}
 y=\frac{\xi}{r},\qquad d=8\pi R^2\Delta_LP_r,
 \qquad q=\left(\frac{\omega R}{c_{\rm light}}\right)^2.
 \label{rpnum:variables}
\end{equation}
Primes in this section denote differentiation with respect to $x$.
Linearizing the Einstein constraints and radial stress-energy conservation,
including the metric perturbations, gives
\begin{align}
 y'&=a_y y+B_d d,\label{rpnum:displacement-equation}\\
 d'&=(C_y+qW_y)y+E_d d,\label{rpnum:pressure-equation}
\end{align}
where
\begin{align}
 a_y&=\frac{\nu'}2-\frac3x-\frac{2\sigma}{wx},\nonumber\\
 B_d&=-\frac{1}{\eta wx},\label{rpnum:coefficients-ab}\\
 C_y&=-4p'-\frac{wpx}{H}+\frac{xw\nu'^2}{4}
       +\frac{2\sigma}{x}\nonumber\\
    &\quad+2\sigma\nu'-\frac{4\sigma^2}{wx},\nonumber\\
 W_y&=\frac{wx}{Hb},\label{rpnum:coefficients-cw}\\
 E_d&=-\frac{\nu'}2-\frac{wx}{2H}
       +\frac{2[\kappa(1+\eta)-1]\sigma}{\eta wx}.
 \label{rpnum:coefficient-e}
\end{align}
For example, the metric constraints used in this reduction are
\begin{align}
 \delta\lambda&=-\frac{x^2wy}{H},\nonumber\\
 \delta\nu'&=\left(\nu'+\frac1x\right)\delta\lambda
                +\frac{x\,\delta p}{H},
 \label{rpnum:metric-constraints}
\end{align}
with $\delta p=d-xyp'$ and
$\delta\varepsilon=d/\eta-xy\varepsilon'$. The anisotropy perturbation is
\begin{equation}
 \delta\sigma=\frac{\kappa(1+\eta)\sigma}{\eta w}d-xy\sigma'.
 \label{rpnum:eulerian-anisotropy}
\end{equation}
Thus the calculation does not freeze the metric or infer a dynamical
anisotropy law from the ratio $P_t'/\rho'$ of the equilibrium profiles.

\subsection{Boundary conditions and spectral problem}
\label{rpnum:boundary-conditions}

Regularity at the center fixes the relation between the two perturbation
variables. Choosing the arbitrary linear normalization $y(0)=1$ gives
\begin{equation}
 d(0)=-3\eta w(0),\qquad \xi(0)=0.
 \label{rpnum:center}
\end{equation}
The regular even-power expansion through $x^6$ supplies initial data close
to the center; it is used only to start the integration. The surface moves
with the fluid, and the appropriate free-boundary condition is
\begin{equation}
 \Delta_LP_r(R)=0,\qquad\hbox{or equivalently}\qquad d(1)=0.
 \label{rpnum:surface}
\end{equation}
Neither $\delta P_r(R)=0$ at fixed radius nor $P_t(R)=0$ is imposed.
For the response law above, Eq.~\eqref{rpnum:surface} also implies
$\Delta_L\rho(R)=\Delta_L\Sigma(R)=0$. The nonzero equilibrium surface
density therefore causes no singular coefficient: although
$\Gamma_r=\eta(\rho+P_r)/P_r$ diverges as $P_r\to0$, the combination
$\Gamma_rP_r=\eta(\rho+P_r)$ entering the equations remains finite.

Eliminating $d$ yields
\begin{equation}
 y''=A_2y'+(V_0-qV_1)y,
 \label{rpnum:second-order}
\end{equation}
where
\begin{align}
 A_2&=a_y+E_d+B_d'/B_d,\nonumber\\
 V_0&=a_y'+B_dC_y-a_y(E_d+B_d'/B_d),\nonumber\\
 V_1&=-B_dW_y=\frac{1}{\eta Hb}>0.
 \label{rpnum:sl-coefficients}
\end{align}
With $\mathcal P=\exp[-\int A_2\,dx]>0$,
$\mathcal Q=\mathcal P V_0$ and $\mathcal W=\mathcal P V_1$, this becomes
\begin{equation}
 - (\mathcal P y')'+\mathcal Qy=q\mathcal Wy.
 \label{rpnum:sturm-liouville}
\end{equation}
Here $\mathcal P\sim x^4$ at the center; the irregular solution
$y\sim x^{-3}$ is excluded. At the surface,
$y'(1)=a_y(1)y(1)$. Accordingly, the Rayleigh quotient includes the
surface term,
\begin{equation}
 q=\frac{\displaystyle\int_0^1
       (\mathcal P y'^2+\mathcal Qy^2)\,dx
       -\mathcal P(1)a_y(1)y(1)^2}
       {\displaystyle\int_0^1\mathcal Wy^2\,dx}.
 \label{rpnum:rayleigh}
\end{equation}
For this real conservative problem, the fundamental mode is nodeless.
The condition $q_0>0$ implies linear radial stability under the specified
closure, whereas $q_0<0$ corresponds to exponential growth.



\subsection{Numerical spectra and mode profiles}
\label{rpnum:results}
\label{section-results}

We computed the fundamental mode and the first three radial overtones for
each of the twelve backgrounds and both values of $\kappa$, obtaining
96 eigenvalues. A continuous Pr\"ufer-phase search includes the negative
$q$ region and is followed by shooting refinement of
Eqs.~\eqref{rpnum:displacement-equation} and \eqref{rpnum:pressure-equation}.
For every background and closure, positivity checks with exact rational
Bernstein coefficients establish $V_0/V_1+100\geq0$ on $0\leq x\leq1$,
and $a_y(1)\leq0$. Equation~\eqref{rpnum:rayleigh} then gives the lower
bound $q\geq-100$, which sets the lower end of the spectral search.

The displacement eigenfunctions have respectively zero, one, two and three
interior nodes. Changing arithmetic precision and the central starting
point changes the eigenvalues by less than $2.4\times10^{-17}$ in the
recorded comparisons. The maximum normalized surface residual is
$6.0\times10^{-23}$; agreement with the Rayleigh quotient and the maximum
normalized overlap of distinct modes are better than
$2.8\times10^{-18}$ and $5.1\times10^{-18}$, respectively. An independent
implementation of the linearized Einstein and conservation equations
agrees within $5.7\times10^{-14}$. The latter refines the previously
located roots and is not an independent global spectral search. These
figures quantify numerical consistency, not physical uncertainty or
rigorous interval bounds on the eigenvalues.

Table~\ref{rpnum:fundamentals} and the fundamental-mode figures below
give the fundamental eigenvalues. All 24 background--closure combinations
have $q_0>0$. Within each sampled family and each closure, $q_0$ decreases
as $u$ increases. The smallest value is $q_0=0.09244687$ for
$\eta=1/4$, $u=0.241$ and $\kappa=0$; its sign remains positive.
The effect of changing the material response is not universal:
$\kappa=1$ lowers $q_0$ in the sampled $\eta=1,1/2,1/3$ families,
whereas for $\eta=1/4$ it lowers $q_0$ at $u=0.158$ and raises it at
$u=0.200$ and $0.241$. No stability boundary is extrapolated from
these three-point samples.

\begin{table}[t]
 \centering
 \caption{Fundamental eigenvalue $q_0=(\omega_0R/c_{\rm light})^2$
 for the twelve equilibrium configurations and the two material
 responses in Eq.~\eqref{rpnum:material-law}.}
 \label{rpnum:fundamentals}
 \begin{tabular}{cccc}
 \hline
 $\eta$ & $u$ & $q_0\ (\kappa=0)$ & $q_0\ (\kappa=1)$\\
 \hline
 $1$   & 0.100 & 5.89513198 & 5.72364703\\
 $1$   & 0.148 & 4.28679684 & 4.05634429\\
 $1$   & 0.196 & 2.87569435 & 2.60583884\\
 $1/2$ & 0.227 & 0.82625953 & 0.70995096\\
 $1/2$ & 0.243 & 0.62339139 & 0.51179733\\
 $1/2$ & 0.259 & 0.43076829 & 0.32740594\\
 $1/3$ & 0.181 & 0.85825179 & 0.81078068\\
 $1/3$ & 0.213 & 0.53611931 & 0.49416880\\
 $1/3$ & 0.244 & 0.25342893 & 0.22409548\\
 $1/4$ & 0.158 & 0.74799673 & 0.73940730\\
 $1/4$ & 0.200 & 0.39547955 & 0.39700572\\
 $1/4$ & 0.241 & 0.09244687 & 0.11232334\\
 \hline
 \end{tabular}
\end{table}

The computed positivity of $q_0$ establishes stability against the radial
perturbations defined above, but it does not establish stability for an
arbitrary anisotropic material law. In particular, it does not remove
the equilibrium limitations associated with the $\eta=1$ family or justify
regions of tangential tension as a microscopic model of quark matter.
Nonradial stability, full characteristic causality and observational
viability require additional analysis. Moreover, the response laws are
constructed around each background; the sampled models are not by
themselves a continuous sequence with a single globally specified
material law. We therefore do not replace the eigenvalue calculation by
a mass-turning-point argument.

Finally, the exterior matching fixes the time normalization. Once a
physical radius is specified, the corresponding cyclic frequency is
\begin{equation}
 f=\frac{c_{\rm light}}{2\pi R}\sqrt q.
 \label{rpnum:frequency-scale}
\end{equation}
The radius also fixes the density scale through $8\pi R^2\rho_s$ in
geometrized units. We therefore report dimensionless eigenvalues and do
not assign a frequency in kilohertz without specifying that scale.

The following individual figures display all 96 modes, with displacement
and Lagrangian pressure perturbation shown separately. Each curve is divided
by its own maximum absolute value over the stored radial grid, so that the
figures compare radial shapes rather than amplitudes:
\begin{equation}
 \widehat\xi=\frac{\xi}{\max|\xi|},\qquad
 \widehat{\Delta_LP_r}=\frac{\Delta_LP_r}{\max|\Delta_LP_r|}.
 \label{rpnum:display-normalization}
\end{equation}
The common integration normalization is $y(0)=1$; the amplitude of a linear
eigenmode remains arbitrary. The absolute displacement vanishes at the
center, while the Lagrangian pressure perturbation vanishes at the surface.
The additional displacement nodes distinguish the three overtones from
the fundamental mode. Each mode profile is drawn as a solid colored line.

For $\eta=1$, the individual profiles in
Figs.~\ref{rpnum:e1-k0-u1-displacement}--\ref{rpnum:e1-k1-u3-pressure}
retain the stiff family as a formal comparison. Both material responses
give positive fundamental eigenvalues at the three compactnesses shown.
The spectral result does not remove the physical reservations about this
equilibrium family discussed above.

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{fundamental_eta_1.pdf}
 \caption{Fundamental radial eigenvalue $q_0$ for $\eta=1$ and
 $\kappa=0,1$. Solid lines join the three computed points as visual
 guides, without defining a continuously calculated sequence.}
 \label{rpnum:fundamental-eta1}
\end{figure}

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{fundamental_eta_3.pdf}
 \caption{Fundamental radial eigenvalue $q_0$ for $\eta=1/3$ and
 $\kappa=0,1$. Solid lines join the three computed points as visual
 guides, without defining a continuously calculated sequence.}
 \label{rpnum:fundamental-eta3}
\end{figure}


\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{fundamental_eta_2.pdf}
 \caption{Fundamental radial eigenvalue $q_0$ for $\eta=1/2$ and
 $\kappa=0,1$. Solid lines join the three computed points as visual
 guides, without defining a continuously calculated sequence.}
 \label{rpnum:fundamental-eta2}
\end{figure}


\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{fundamental_eta_4.pdf}
 \caption{Fundamental radial eigenvalue $q_0$ for $\eta=1/4$ and
 $\kappa=0,1$. Solid lines join the three computed points as visual
 guides, without defining a continuously calculated sequence.}
 \label{rpnum:fundamental-eta4}
\end{figure}












\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e1-k0-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k0-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e1-k0-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k0-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e1-k0-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k0-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_0_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1$ and $\kappa=0$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.100$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.148$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.196$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e1-k0-modes}
\end{figure*}

\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e1-k1-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k1-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e1-k1-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k1-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e1-k1-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e1-k1-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_1_kappa_1_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1$ and $\kappa=1$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.100$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.148$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.196$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e1-k1-modes}
\end{figure*}

For $\eta=1/2$, Figs.~\ref{rpnum:e2-k0-u1-displacement}--\ref{rpnum:e2-k1-u3-pressure}
show the displacement and pressure response at $u=0.227,0.243,0.259$.
The fundamental eigenvalue remains positive and decreases across these
sampled compactnesses for both closures. Changing the closure also changes
the eigenfunctions, even though the equilibrium is held fixed.



\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e2-k0-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k0-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e2-k0-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k0-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e2-k0-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k0-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_0_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/2$ and $\kappa=0$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.227$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.243$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.259$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e2-k0-modes}
\end{figure*}

\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e2-k1-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k1-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e2-k1-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k1-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e2-k1-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e2-k1-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_2_kappa_1_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/2$ and $\kappa=1$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.227$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.243$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.259$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e2-k1-modes}
\end{figure*}

For $\eta=1/3$, Figs.~\ref{rpnum:e3-k0-u1-displacement}--\ref{rpnum:e3-k1-u3-pressure}
show all four modes at $u=0.181,0.213,0.244$. The displacement profiles
exhibit the expected progression from the nodeless fundamental mode to
three nodes in the third overtone. The surface condition applies to the
Lagrangian pressure perturbation in each of the accompanying profiles.




\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e3-k0-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k0-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e3-k0-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k0-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e3-k0-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k0-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_0_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/3$ and $\kappa=0$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.181$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.213$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.244$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e3-k0-modes}
\end{figure*}

\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e3-k1-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k1-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e3-k1-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k1-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e3-k1-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e3-k1-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_3_kappa_1_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/3$ and $\kappa=1$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.181$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.213$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.244$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e3-k1-modes}
\end{figure*}

For $\eta=1/4$, Figs.~\ref{rpnum:e4-k0-u1-displacement}--\ref{rpnum:e4-k1-u3-pressure}
complete the mode comparison at $u=0.158,0.200,0.241$. This family contains
the smallest computed fundamental eigenvalue. Both closures still give
$q_0>0$, while their ordering changes between the lowest and the two
higher sampled compactnesses.



\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e4-k0-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k0-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e4-k0-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k0-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e4-k0-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k0-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_0_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/4$ and $\kappa=0$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.158$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.200$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.241$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e4-k0-modes}
\end{figure*}

\begin{figure*}[!t]
\centering
\subfloat[\label{rpnum:e4-k1-u1-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_1_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k1-u1-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_1_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e4-k1-u2-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_2_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k1-u2-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_2_pressure.pdf}
}
\par\medskip
\subfloat[\label{rpnum:e4-k1-u3-displacement}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_3_displacement.pdf}
}
\hfill
\subfloat[\label{rpnum:e4-k1-u3-pressure}]{%
  \includegraphics[width=0.49\textwidth]{pulse_eta_4_kappa_1_u_3_pressure.pdf}
}
\caption{Normalized radial modes for $\eta=1/4$ and $\kappa=1$. (a) $\widehat{\xi}$ and (b) $\widehat{\Delta_LP_r}$ for $u=0.158$; (c) $\widehat{\xi}$ and (d) $\widehat{\Delta_LP_r}$ for $u=0.200$; (e) $\widehat{\xi}$ and (f) $\widehat{\Delta_LP_r}$ for $u=0.241$. Each panel shows modes $j=0,1,2,3$ as solid colored curves, normalized separately as in Eq.~\eqref{rpnum:display-normalization}.}
\label{rpnum:e4-k1-modes}
\end{figure*}

%\FloatBarrier


==> pulsations_section.tex <==
\section{Radial pulsations of the self-bound configurations}
\label{rpnum:section}

We now investigate the linear radial response of the twelve equilibrium
configurations considered above. A static anisotropy profile does not specify
how the anisotropic stress responds to a displacement of the fluid. We therefore
state the material response explicitly and compare two closures that reproduce
the same equilibrium. The resulting stability statements refer to these
closures. This distinction is particularly relevant when the tangential
pressure remains nonzero at the surface, as in radial-stability studies of
anisotropic strange stars~\cite{arbanil2016anisotropic}.

\subsection{Material response and perturbation equations}
\label{rpnum:closure}

Let $\xi(r)e^{i\omega t}$ denote the radial displacement and let $\Delta_L$
and $\delta$ denote Lagrangian and Eulerian perturbations, respectively, so
that $\Delta_L F=\delta F+\xi\,dF/dr$. The equilibrium parameters $\eta$ and
$\rho_s$ are held fixed during each oscillation. Consequently,
\begin{equation}
 \Delta_L P_r=\eta\,\Delta_L\rho.
 \label{rpnum:perturbed-eos}
\end{equation}
Writing $\Sigma=P_t-P_r$ for the physical anisotropy, we introduce a material
label $a_L$ that is transported with each fluid layer and prescribe
\begin{equation}
 \Sigma(a_L,\rho)=\Sigma_0(a_L)
 \left[\frac{\rho+P_r}{\rho_0(a_L)+P_{r0}(a_L)}\right]^\kappa,
 \qquad \kappa=0,1.
 \label{rpnum:material-law}
\end{equation}
The subscript $0$ denotes the chosen background. For $\kappa=0$, each layer
preserves its anisotropy, whereas for $\kappa=1$ it preserves
$\Sigma/(\rho+P_r)$. These are phenomenological response laws; they are not
deduced from the equilibrium equation of state or from gravitational
decoupling. Both preserve the central behavior $\Sigma=O(r^2)$ on the regular
perturbative branch. Their linearization gives
\begin{equation}
 \Delta_L\Sigma=
 \frac{\kappa(1+\eta)\Sigma}{\eta(\rho+P_r)}\Delta_LP_r.
 \label{rpnum:anisotropy-response}
\end{equation}
In particular, $\Delta_L\Sigma=0$ and $\delta\Sigma=0$ are different
prescriptions.

For the numerical problem we use $x=r/R$, $H=e^{-\lambda}$,
$b=e^\nu=1-3u+ux^2$, and the dimensionless background variables
\begin{equation}
 \begin{aligned}
 \varepsilon&=8\pi R^2\rho,& p&=8\pi R^2P_r,\\
 \sigma&=8\pi R^2(P_t-P_r),& w&=\varepsilon+p.
 \end{aligned}
 \label{rpnum:background-variables}
\end{equation}
The factors in Eq.~\eqref{rpnum:background-variables} use geometrized units,
$G=c_{\rm light}=1$. We define
\begin{equation}
 y=\frac{\xi}{r},\qquad d=8\pi R^2\Delta_LP_r,
 \qquad q=\left(\frac{\omega R}{c_{\rm light}}\right)^2.
 \label{rpnum:variables}
\end{equation}
Primes in this section denote differentiation with respect to $x$.
Linearizing the Einstein constraints and radial stress-energy conservation,
including the metric perturbations, gives
\begin{align}
 y'&=a_y y+B_d d,\label{rpnum:displacement-equation}\\
 d'&=(C_y+qW_y)y+E_d d,\label{rpnum:pressure-equation}
\end{align}
where
\begin{align}
 a_y&=\frac{\nu'}2-\frac3x-\frac{2\sigma}{wx},\nonumber\\
 B_d&=-\frac{1}{\eta wx},\label{rpnum:coefficients-ab}\\
 C_y&=-4p'-\frac{wpx}{H}+\frac{xw\nu'^2}{4}
       +\frac{2\sigma}{x}\nonumber\\
    &\quad+2\sigma\nu'-\frac{4\sigma^2}{wx},\nonumber\\
 W_y&=\frac{wx}{Hb},\label{rpnum:coefficients-cw}\\
 E_d&=-\frac{\nu'}2-\frac{wx}{2H}
       +\frac{2[\kappa(1+\eta)-1]\sigma}{\eta wx}.
 \label{rpnum:coefficient-e}
\end{align}
For example, the metric constraints used in this reduction are
\begin{align}
 \delta\lambda&=-\frac{x^2wy}{H},\nonumber\\
 \delta\nu'&=\left(\nu'+\frac1x\right)\delta\lambda
                +\frac{x\,\delta p}{H},
 \label{rpnum:metric-constraints}
\end{align}
with $\delta p=d-xyp'$ and
$\delta\varepsilon=d/\eta-xy\varepsilon'$. The anisotropy perturbation is
\begin{equation}
 \delta\sigma=\frac{\kappa(1+\eta)\sigma}{\eta w}d-xy\sigma'.
 \label{rpnum:eulerian-anisotropy}
\end{equation}
Thus the calculation does not freeze the metric or infer a dynamical
anisotropy law from the ratio $P_t'/\rho'$ of the equilibrium profiles.

\subsection{Boundary conditions and spectral problem}
\label{rpnum:boundary-conditions}

Regularity at the center fixes the relation between the two perturbation
variables. Choosing the arbitrary linear normalization $y(0)=1$ gives
\begin{equation}
 d(0)=-3\eta w(0),\qquad \xi(0)=0.
 \label{rpnum:center}
\end{equation}
The regular even-power expansion through $x^6$ supplies initial data close
to the center; it is used only to start the integration. The surface moves
with the fluid, and the appropriate free-boundary condition is
\begin{equation}
 \Delta_LP_r(R)=0,\qquad\hbox{or equivalently}\qquad d(1)=0.
 \label{rpnum:surface}
\end{equation}
Neither $\delta P_r(R)=0$ at fixed radius nor $P_t(R)=0$ is imposed.
For the response law above, Eq.~\eqref{rpnum:surface} also implies
$\Delta_L\rho(R)=\Delta_L\Sigma(R)=0$. The nonzero equilibrium surface
density therefore causes no singular coefficient: although
$\Gamma_r=\eta(\rho+P_r)/P_r$ diverges as $P_r\to0$, the combination
$\Gamma_rP_r=\eta(\rho+P_r)$ entering the equations remains finite.

Eliminating $d$ yields
\begin{equation}
 y''=A_2y'+(V_0-qV_1)y,
 \label{rpnum:second-order}
\end{equation}
where
\begin{align}
 A_2&=a_y+E_d+B_d'/B_d,\nonumber\\
 V_0&=a_y'+B_dC_y-a_y(E_d+B_d'/B_d),\nonumber\\
 V_1&=-B_dW_y=\frac{1}{\eta Hb}>0.
 \label{rpnum:sl-coefficients}
\end{align}
With $\mathcal P=\exp[-\int A_2\,dx]>0$,
$\mathcal Q=\mathcal P V_0$ and $\mathcal W=\mathcal P V_1$, this becomes
\begin{equation}
 - (\mathcal P y')'+\mathcal Qy=q\mathcal Wy.
 \label{rpnum:sturm-liouville}
\end{equation}
Here $\mathcal P\sim x^4$ at the center; the irregular solution
$y\sim x^{-3}$ is excluded. At the surface,
$y'(1)=a_y(1)y(1)$. Accordingly, the Rayleigh quotient includes the
surface term,
\begin{equation}
 q=\frac{\displaystyle\int_0^1
       (\mathcal P y'^2+\mathcal Qy^2)\,dx
       -\mathcal P(1)a_y(1)y(1)^2}
       {\displaystyle\int_0^1\mathcal Wy^2\,dx}.
 \label{rpnum:rayleigh}
\end{equation}
For this real conservative problem, the fundamental mode is nodeless.
The condition $q_0>0$ implies linear radial stability under the specified
closure, whereas $q_0<0$ corresponds to exponential growth.

\subsection{Numerical spectra and mode profiles}
\label{rpnum:results}

We computed the fundamental mode and the first three radial overtones for
each of the twelve backgrounds and both values of $\kappa$, obtaining
96 eigenvalues. A continuous Pr\"ufer-phase search includes the negative
$q$ region and is followed by shooting refinement of
Eqs.~\eqref{rpnum:displacement-equation}--\eqref{rpnum:pressure-equation}.
For every background and closure, positivity checks with exact rational
Bernstein coefficients establish $V_0/V_1+100\geq0$ on $0\leq x\leq1$,
and $a_y(1)\leq0$. Equation~\eqref{rpnum:rayleigh} then gives the lower
bound $q\geq-100$, which sets the lower end of the spectral search.

The displacement eigenfunctions have respectively zero, one, two and three
interior nodes. Changing arithmetic precision and the central starting
point changes the eigenvalues by less than $2.4\times10^{-17}$ in the
recorded comparisons. The maximum normalized surface residual is
$6.0\times10^{-23}$; agreement with the Rayleigh quotient and the maximum
normalized overlap of distinct modes are better than
$2.8\times10^{-18}$ and $5.1\times10^{-18}$, respectively. An independent
implementation of the linearized Einstein and conservation equations
agrees within $5.7\times10^{-14}$. The latter refines the previously
located roots and is not an independent global spectral search. These
figures quantify numerical consistency, not physical uncertainty or
rigorous interval bounds on the eigenvalues.

Table~\ref{rpnum:fundamentals} and Fig.~\ref{rpnum:fundamental-figure}
give the fundamental eigenvalues. All 24 background--closure combinations
have $q_0>0$. Within each sampled family and each closure, $q_0$ decreases
as $u$ increases. The smallest value is $q_0=0.09244687$ for
$\eta=1/4$, $u=0.241$ and $\kappa=0$; its sign remains positive.
The effect of changing the material response is not universal:
$\kappa=1$ lowers $q_0$ in the sampled $\eta=1,1/2,1/3$ families,
whereas for $\eta=1/4$ it lowers $q_0$ at $u=0.158$ and raises it at
$u=0.200$ and $0.241$. No stability boundary is extrapolated from
these three-point samples.

\begin{table}[t]
 \centering
 \caption{Fundamental eigenvalue $q_0=(\omega_0R/c_{\rm light})^2$
 for the twelve equilibrium configurations and the two material
 responses in Eq.~\eqref{rpnum:material-law}.}
 \label{rpnum:fundamentals}
 \begin{tabular}{cccc}
 \hline
 $\eta$ & $u$ & $q_0\ (\kappa=0)$ & $q_0\ (\kappa=1)$\\
 \hline
 $1$   & 0.100 & 5.89513198 & 5.72364703\\
 $1$   & 0.148 & 4.28679684 & 4.05634429\\
 $1$   & 0.196 & 2.87569435 & 2.60583884\\
 $1/2$ & 0.227 & 0.82625953 & 0.70995096\\
 $1/2$ & 0.243 & 0.62339139 & 0.51179733\\
 $1/2$ & 0.259 & 0.43076829 & 0.32740594\\
 $1/3$ & 0.181 & 0.85825179 & 0.81078068\\
 $1/3$ & 0.213 & 0.53611931 & 0.49416880\\
 $1/3$ & 0.244 & 0.25342893 & 0.22409548\\
 $1/4$ & 0.158 & 0.74799673 & 0.73940730\\
 $1/4$ & 0.200 & 0.39547955 & 0.39700572\\
 $1/4$ & 0.241 & 0.09244687 & 0.11232334\\
 \hline
 \end{tabular}
\end{table}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{fundamental_modes.pdf}
 \caption{Fundamental radial eigenvalues for the four values of $\eta$.
 Each panel compares the two material responses at the same three
 equilibrium compactnesses. Solid lines join computed points as visual
 guides; they do not represent a continuously calculated sequence or
 establish a turning point.}
 \label{rpnum:fundamental-figure}
\end{figure*}

Figures~\ref{rpnum:eta1-k0}--\ref{rpnum:eta4-k1} display all 96 modes,
with displacement and Lagrangian pressure perturbation shown separately.
Each curve is divided by its own maximum absolute value over the stored
radial grid, so that the figures compare radial shapes rather than
amplitudes. The common integration normalization is $y(0)=1$; the
amplitudes of a linear eigenmode remain arbitrary. The vanishing absolute
displacement at the center and the vanishing Lagrangian pressure
perturbation at the surface are manifest in the profiles. The additional
displacement nodes distinguish the three overtones from the fundamental
mode. All curves use solid colored lines.

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_1_kappa_0.pdf}
 \caption{Radial modes for $\eta=1$ and $\kappa=0$, retained as a formal
 comparison. Rows correspond to $u=0.100,0.148,0.196$.
 The left column shows $\widehat\xi=\xi/\max|\xi|$ and the right column
 $\widehat{\Delta_LP_r}=\Delta_LP_r/\max|\Delta_LP_r|$.
 Each panel contains modes $0,1,2,3$, identified by color. Each curve is
 normalized separately; extrema for this display are taken over the
 stored radial grid.}
 \label{rpnum:eta1-k0}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_1_kappa_1.pdf}
 \caption{Radial modes for $\eta=1$ and $\kappa=1$, retained as a formal
 comparison. Rows correspond to $u=0.100,0.148,0.196$; columns and
 normalization are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta1-k1}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_2_kappa_0.pdf}
 \caption{Radial modes for $\eta=1/2$ and $\kappa=0$.
 Rows correspond to $u=0.227,0.243,0.259$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta2-k0}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_2_kappa_1.pdf}
 \caption{Radial modes for $\eta=1/2$ and $\kappa=1$.
 Rows correspond to $u=0.227,0.243,0.259$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta2-k1}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_3_kappa_0.pdf}
 \caption{Radial modes for $\eta=1/3$ and $\kappa=0$.
 Rows correspond to $u=0.181,0.213,0.244$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta3-k0}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_3_kappa_1.pdf}
 \caption{Radial modes for $\eta=1/3$ and $\kappa=1$.
 Rows correspond to $u=0.181,0.213,0.244$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta3-k1}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_4_kappa_0.pdf}
 \caption{Radial modes for $\eta=1/4$ and $\kappa=0$.
 Rows correspond to $u=0.158,0.200,0.241$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta4-k0}
\end{figure*}

\begin{figure*}[p]
 \centering
 \includegraphics[width=0.94\textwidth,height=0.75\textheight,keepaspectratio]{pulsations_eta_4_kappa_1.pdf}
 \caption{Radial modes for $\eta=1/4$ and $\kappa=1$.
 Rows correspond to $u=0.158,0.200,0.241$; columns and normalization
 are as in Fig.~\ref{rpnum:eta1-k0}.}
 \label{rpnum:eta4-k1}
\end{figure*}

The computed positivity of $q_0$ establishes stability against the radial
perturbations defined above, but it does not establish stability for an
arbitrary anisotropic material law. In particular, it does not remove the
equilibrium limitations associated with the $\eta=1$ family or justify
regions of tangential tension as a microscopic model of quark matter.
Nonradial stability, full characteristic causality and observational
viability require additional analysis. Moreover, the response laws are
constructed around each background; the sampled models are not by
themselves a continuous sequence with a single globally specified
material law. We therefore do not replace the eigenvalue calculation by
a mass-turning-point argument.

Finally, the exterior matching fixes the time normalization. Once a
physical radius is specified, the corresponding cyclic frequency is
\begin{equation}
 f=\frac{c_{\rm light}}{2\pi R}\sqrt q.
 \label{rpnum:frequency-scale}
\end{equation}
The radius also fixes the density scale through $8\pi R^2\rho_s$ in
geometrized units. We therefore report dimensionless eigenvalues and do
not assign a frequency in kilohertz without specifying that scale.

\clearpage

